SE-Sync: A Certifiably Correct Algorithm for Synchronization over the Special Euclidean Group

Many important geometric estimation problems take the form of synchronization over the special Euclidean group: estimate the values of a set of poses given a set of relative measurements between them. This problem is typically formulated as a nonconvex maximum-likelihood estimation that is computationally hard to solve in general. Nevertheless, in this paper we present an algorithm that is able to efficiently recover certifiably globally optimal solutions of the special Euclidean synchronization problem in a non-adversarial noise regime. The crux of our approach is the development of a semidefinite relaxation of the maximum-likelihood estimation whose minimizer provides an exact MLE so long as the magnitude of the noise corrupting the available measurements falls below a certain critical threshold; furthermore, whenever exactness obtains, it is possible to verify this fact a posteriori, thereby certifying the optimality of the recovered estimate. We develop a specialized optimization scheme for solving large-scale instances of this relaxation by exploiting its low-rank, geometric, and graph-theoretic structure to reduce it to an equivalent optimization problem on a low-dimensional Riemannian manifold, and design a truncated-Newton trust-region method to solve this reduction efficiently. Finally, we combine this fast optimization approach with a simple rounding procedure to produce our algorithm, SE-Sync. Experimental evaluation on a variety of simulated and real-world pose-graph SLAM datasets shows that SE-Sync is able to recover certifiably globally optimal solutions when the available measurements are corrupted by noise up to an order of magnitude greater than that typically encountered in robotics and computer vision applications, and does so more than an order of magnitude faster than the Gauss-Newton-based approach that forms the basis of current state-of-the-art techniques.

==> Cycle_spaces_and_cycle_bases.tex <==
\section{The cycle space of a graph}
\label{cycle_spaces_appendix}

In this section we briefly introduce the notion of the cycle space associated with a graph; interested readers are directed to \cite{Biggs1997Algebraic,Kavitha2009Cycle} for additional detail.

\subsection{Definition}

Let $\directed{G} = (\Nodes, \dEdges)$ be a directed graph with $n = \lvert \Nodes \rvert$ and $m = \lvert \dEdges \rvert$ and $\F$ be a field.  We may associate to $\directed{G}$ the free $\F$-vector spaces $\chain_1(\directed{G}; \F)$ and $\chain_0(\directed{G}; \F)$ consisting of all formal $\F$-linear sums of $\directed{G}$'s edges and vertices, respectively:
\begin{equation}
\label{vector_spaces}
\chain_1(\directed{G}; \F) \triangleq \left \lbrace \sum_{e \in \dEdges} c_e e \mid c_e \in \F \right \rbrace \cong \F^m, \quad \quad \chain_0(\directed{G}; \F) \triangleq \left \lbrace \sum_{v \in \Nodes} c_v v \mid c_v \in \F \right \rbrace \cong \F^n, 
\end{equation}
and define a corresponding \emph{boundary operator} $\partial_1 \colon \chain_1(\directed{G}; \F) \to \chain_0(\directed{G}; \F)$ between them as the unique linear extension of the assignment $\partial_1( v,w ) \triangleq w - v$ that maps each directed edge $(v,w) \in \dEdges$ to its (oriented) endpoints: 
\begin{equation}
\label{edge_boundary_operator_definition}
\begin{split}
\partial_1 &\colon \chain_1(\directed{G}; \F) \to \chain_0(\directed{G}; \F) \\
\partial_1\left( \sum_{e \in \dEdges} c_e e \right) &= \sum_{v \in \Nodes} \left( \sum_{e \in \inEdges(v)} c_e - \sum_{e \in \outEdges(v)} c_e \right) v.
\end{split}
\end{equation}
We denote the kernel of $\partial_1$ by $\cycSpace(\directed{G}; \F)$; it follows from \eqref{edge_boundary_operator_definition} that this subspace is given explicitly by:
\begin{equation}
 \label{cycle_space_definition}
\cycSpace(\directed{G}; \F) \triangleq \ker(\partial_1) = \left \lbrace \sum_{e \in \dEdges} c_e e \mid \sum_{e \in \inEdges(v)} c_e = \sum_{e \in \outEdges(v)} c_e \quad \forall v \in \Nodes  \right \rbrace \subseteq \chain_1(\directed{G}; \F).
\end{equation}

If we interpret each edge $e = \dedge \in \dEdges$ as the pathway for a flow from vertex $i$ to vertex $j$, and its associated coefficient $c_e \in \F$ as the (directed) magnitude of that flow, then the condition appearing in \eqref{cycle_space_definition} is simply the requirement that the net flows into and out of each vertex $v \in \Nodes$ must be equal; we refer to this condition as \emph{flow conservation}, and (in consequence) to the elements $z \in \cycSpace(\directed{G}; \F)$ as \emph{flows} or ($\F$-)\emph{cycles}.  The subspace $\cycSpace(\directed{G}; \F) \subseteq \chain_1(\directed{G} ; \F)$ itself is called the $\F$-\emph{cycle space} of $\directed{G}$.\footnote{Readers who are familiar with simplicial homology will also recognize $\cycSpace(\directed{G}; \F)$ as $H_1(\directed{G}; \F)$, the first homology group of $\directed{G}$ considered as a simplicial $1$-complex (hence the use of our highly suggestive choice of notation in equations \eqref{vector_spaces}--\eqref{cycle_space_definition}).}  


The \emph{support} of a cycle in \eqref{cycle_space_definition} is the set of edges $e \in \dEdges$ with $c_e \ne 0$.  A cycle is called \emph{simple} if $c_e \in \lbrace -1, 0, 1 \rbrace$ for all $e \in \dEdges$, and a simple cycle is a \emph{circuit} if its support is weakly connected and for any $v \in \Nodes$ there are at most two edges in the support incident to $v$.  An $\F$-\emph{cycle basis} is a set of circuits forming a basis for the cycle space $\cycSpace(\directed{G}; \F)$. It can be shown that $\dim(\cycSpace(\directed{G}; \F)) = m - n + c$, where $c$ is the number of $\directed{G}$'s weakly-connected components, and that $\cycSpace(\directed{G}; \F)$ always admits a cycle basis (cf.\ \cite[Theorem 2.3]{Kavitha2009Cycle}).\footnote{Note that this latter point is nontrivial: while the linear space $\cycSpace(\directed{G};\F)$ always admits a basis, a \emph{cycle basis} is a basis satisfying additional constraints.}  Consequently, we let $\nu \triangleq m - n + c$, and refer to this quantity as $\directed{G}$'s \emph{cyclomatic number}.  

We can generalize this construction to an undirected graph $G$ by considering the cycle space of one of its orientations $\directed{G}$.  If $\directed{G}$ and $\directed{G}'$ are two orientations of $G$, then the cycle spaces $\cycSpace(\directed{G}; \F)$ and $\cycSpace(\directed{G}'; \F)$ are isomorphic under the mapping $\psi \colon \cycSpace(\directed{G}; \F)\to \cycSpace(\directed{G}'; \F)$ that reverses the sign of the scalars $c_e$ in \eqref{cycle_space_definition} corresponding to edges $e$ that are oriented differently in $\directed{G}$ and $\directed{G}'$.  Consequently, the isomorphism class of the cycle space $\cycSpace(\directed{G}; \F)$ associated to $G$ in this way does not actually depend upon the specific orientation $\directed{G}$ selected (i.e.\ it is determined by the underlying graph $G$ itself), and we are therefore justified in defining $\cycSpace(G; \F) \triangleq \cycSpace(\directed{G}; \F)$ and referring to $\cycSpace(G; \F)$ as the \emph{cycle space} of $G$.

The most common choices of the field $\F$ are $\F = \Q$ and $\F = \Z_2$ (the two-element finite field); in these cases, the cycle spaces and bases are referred to as \emph{directed} and \emph{undirected}, respectively.

\subsection{Computing the orthogonal projection matrix}
\label{Computing_the_orthogonal_projection_matrix_subsection}
In this subsection we describe two methods for computing the matrix of the orthogonal projection operator onto the directed cycle space of a weakly connected graph.

Let $\directed{G} = (\Nodes, \dEdges)$ be a weakly connected directed graph, $\F = \R$, and fix an ordering of the edges $\dEdges$ and vertices $\Nodes$ (thus providing explicit identifications of $\chain_1(\directed{G}) \triangleq \chain_1(\directed{G}; \R)$ with $\R^m$ and $\chain_0(\directed{G}) \triangleq \chain_0(\directed{G}; \R)$ with $\R^n$).  Given any directed cycle basis $\cycBasis = \lbrace C_1, \dotsc, C_{\nu} \rbrace \subset \Z^m$ for the directed cycle space $\cycSpace(\directed{G}) \triangleq \cycSpace(\directed{G}, \R)$, we can construct the associated \emph{cycle matrix} $\Gamma$:
\begin{equation}
 \label{cycle_matrix_definition}
 \Gamma \triangleq 
 \begin{pmatrix}
C_1 & \dotsb & C_{\nu} 
 \end{pmatrix} \in \Z^{m \times \nu}.
\end{equation}
Since $B$ is a basis for $\cycSpace(\directed{G})$, then $\image(\Gamma) = \cycSpace(\directed{G})$, and consequently the matrix $\OrthoProjMatrix$ of the orthogonal projection operator $\OrthoProj \colon \R^m \to \cycSpace(\directed{G}))$ onto the directed cycle space of $\directed{G}$ is given by \cite[eq.\ (5.13.12)]{Meyer2000Matrix}:
\begin{equation}
\label{matrix_of_orthogonal_projection_operator_onto_cycle_space_in_terms_of_cycle_matrix}
 \OrthoProjMatrix = \cycMat \cycMat\pinv.
\end{equation}

Alternatively, we can also compute $\OrthoProjMatrix$ using the incidence matrix $\incMat(\directed{G})$.  Observe that the matrix of the boundary operator $\partial_1$ in \eqref{edge_boundary_operator_definition} is actually $\incMat(\directed{G})$ itself; to see this, simply note that the $e$th column of $\incMat(\directed{G})$ has a $+1$ in the row corresponding to $h(e)$, a $-1$ in the row corresponding to $t(e)$, and zeros elsewhere.  Therefore, we also have the alternative (although completely equivalent) characterization of $\cycSpace(\directed{G})$ as:
\begin{equation}
\label{cycle_space_is_kernel_of_incidence_matrix}
 \cycSpace(\directed{G}) = \ker(\incMat(\directed{G})) \subseteq \R^m .
\end{equation}
It follows from \eqref{cycle_space_is_kernel_of_incidence_matrix} that $\OrthoProjMatrix$ can also be expressed as (see again \cite[eq.\ (5.13.12)]{Meyer2000Matrix}):
\begin{equation}
\label{matrix_of_orthogonal_projection_operator_onto_cycle_space}
\OrthoProjMatrix = I_m - \incMat(\directed{G})\pinv \incMat(\directed{G}).
\end{equation}

While computing the pseudoinverse of a large matrix is in general an expensive operation, in this case we can exploit the additional knowledge that $\incMat(\directed{G})$ is the incidence matrix of a weakly-connected directed graph to speed up the computation of the product on the right-hand side of \eqref{matrix_of_orthogonal_projection_operator_onto_cycle_space}.  To do so, we will exploit the following lemma:

\begin{lem}
\label{pseudoinverse_of_incidence_matrix_lemma}
 Let $\incMat \in \R^{n \times m}$ be the incidence matrix for a weakly-connected directed graph.  Then the pseudoinverse of $\incMat$ is given by:
 \begin{equation}
 \label{pseudoinverse_of_incidence_matrix_equation}
\incMat\pinv = \redIncMat\transpose \left( \redIncMat \redIncMat\transpose \right)^{-1}
\begin{pmatrix}
 I_{n-1} - \frac{1}{n} \ones_{n-1} \ones_{n-1}\transpose & - \frac{1}{n} \ones_{n-1}
\end{pmatrix}
 \end{equation}
 where $\redIncMat \in \R^{(n-1) \times m}$ is the reduced incidence matrix obtained by removing the final row of $\incMat$.
\end{lem}
\begin{proof}
By definition $\incMat$ has a single instance of $1$ and $-1$ in each of its columns, and therefore $\ones_n\transpose\incMat = 0$.
 We first show that $\incMat$ can be decomposed as follows:
\begin{equation}
\label{eq:decomposeIncMat}
\incMat = 
\begin{pmatrix}
I_{n-1} \\
-\ones_{n-1}\transpose
\end{pmatrix}
\redIncMat.
\end{equation}
Letting $a \in \R^{1 \times m}$ denote the final row of $\incMat$, we observe that
\begin{equation}
 \ones_n\transpose \incMat = \ones_n\transpose 
 \begin{pmatrix}
 \redIncMat \\
 a
 \end{pmatrix}
=
\ones_{n-1}\transpose \redIncMat + a = 0;
\end{equation}
this implies that $a = -\ones_{n-1}\transpose \redIncMat$, which is \eqref{eq:decomposeIncMat}.  Now let $E \triangleq \begin{pmatrix}I_{n-1} & -\ones_{n-1} \end{pmatrix}\transpose$ denote the matrix appearing in \eqref{eq:decomposeIncMat}, and consider:
 \begin{equation}
\label{eq:pinv2}
\incMat\pinv = (E \redIncMat )\pinv =  \redIncMat\pinv E\pinv.
\end{equation}
Since $E$ is full column rank, its pseudoinverse $E\pinv$ is
\begin{equation}
\label{pseudoinverse_of_E}
 E\pinv = \left(E\transpose E \right)^{-1} E\transpose;
\end{equation}
furthermore, observing that
\begin{equation}
\label{setup_to_compute_inverse_of_EEtranspose_using_SM_formula}
\left(E\transpose E \right)^{-1} =
\left(
\begin{pmatrix}
I_{n-1} \\
-\ones_{n-1}\transpose
\end{pmatrix}\transpose
\begin{pmatrix}
I_{n-1} \\
-\ones_{n-1}\transpose
\end{pmatrix}
\right)^{-1}
=
\left( I_{n-1} + \ones_{n-1}\transpose \ones_{n-1} \right)^{-1}
\end{equation}
is the inverse of a rank-1 additive update of $I_{n-1}$, we may apply the Sherman-Morrison formula \cite[eq.\ (2.1.4)]{Golub1996Matrix} to the right-hand side of \eqref{setup_to_compute_inverse_of_EEtranspose_using_SM_formula} to compute:
\begin{equation}
\label{eq:SMformula}
\left (E\transpose E \right)^{-1} =   
I_{n-1} - \frac{I_{n-1} \ones_{n-1}\ones_{n-1}\transpose I_{n-1}  }{ 1 + \ones_{n-1}\transpose I_{n-1} \ones_{n-1} } =
 I_{n-1} - \frac{1}{n} \ones_{n-1}\ones_{n-1}\transpose.
\end{equation}
Substituting~\eqref{eq:SMformula} back into \eqref{pseudoinverse_of_E}, we obtain:
\begin{equation}
\label{simplified_form_of_pseudoinverse_of_E}
\begin{split}
(E\transpose E)^{-1} E\transpose &= \left( I_{n-1} - \frac{1}{n} \ones_{n-1}\ones_{n-1}\transpose \right) 
\begin{pmatrix}
 I_{n-1} \\
 -\ones_{n-1}\transpose
\end{pmatrix}\transpose \\
&= 
\begin{pmatrix}
 I_{n-1} - \frac{1}{n} \ones_{n-1} \ones_{n-1}\transpose & - \frac{1}{n} \ones_{n-1}
\end{pmatrix}.
\end{split}
\end{equation}
Similarly, $\redIncMat$ is full row rank (as it is the reduced incidence matrix of a weakly connected graph), and therefore
\begin{equation}
\label{pseudoinverse_of_reduced_incidence_matrix}
\redIncMat\pinv = \redIncMat\transpose (\redIncMat \redIncMat\transpose)^{-1}.
\end{equation}
Substituting \eqref{simplified_form_of_pseudoinverse_of_E} and \eqref{pseudoinverse_of_reduced_incidence_matrix} into \eqref{eq:pinv2} gives \eqref{pseudoinverse_of_incidence_matrix_equation}.
\end{proof}

Applying Lemma \ref{pseudoinverse_of_incidence_matrix_lemma} and  the decomposition \eqref{eq:decomposeIncMat} for $\incMat(\directed{G})$, the product on the right-hand side of \eqref{matrix_of_orthogonal_projection_operator_onto_cycle_space} can be expanded as:
\begin{equation}
\label{product_in_orthogonal_projection_operator_in_terms_of_reduced_incidence_matrices}
\begin{split}
 \incMat(\directed{G)}\pinv \incMat(\directed{G)} &=\left(\redIncMat(\directed{G})\transpose \left( \redIncMat(\directed{G}) \redIncMat(\directed{G})\transpose \right)^{-1} \begin{pmatrix}
 I_{n-1} - \frac{1}{n} \ones_{n-1} \ones_{n-1}\transpose & - \frac{1}{n} \ones_{n-1}
\end{pmatrix} \right) \left(
\begin{pmatrix}
I_{n-1} \\
-\ones_{n-1}\transpose
\end{pmatrix}
\redIncMat(\directed{G}) \right) \\
&= \redIncMat(\directed{G})\transpose \left(\redIncMat(\directed{G}) \redIncMat(\directed{G})\transpose \right)^{-1} \redIncMat(\directed{G}).
\end{split}
\end{equation}
Furthermore, $\redIncMat(\directed{G})$ is full row rank, as it is the reduced incidence matrix of a weakly-connected directed graph.  Therefore, letting
\begin{equation}
 \redIncMat(\directed{G}) =
 \begin{pmatrix}
 L &  
 0
 \end{pmatrix} Q
\end{equation}
be an LQ decomposition\footnote{This is the transpose of a QR decomposition \cite[Sec.\ 5.2]{Golub1996Matrix}.} of $\redIncMat(\directed{G})$, equation \eqref{product_in_orthogonal_projection_operator_in_terms_of_reduced_incidence_matrices} is equivalent to:
\begin{equation}
\label{product_in_orthogonal_projection_operator_in_terms_of_reduced_incidence_matrices_and_sparse_R_factors}
  \incMat(\directed{G)}\pinv \incMat(\directed{G)} = \redIncMat(\directed{G})\transpose L\tinv L\inv \redIncMat(\directed{G}).
\end{equation}
% The advantage of the right-hand side of equation \eqref{product_in_orthogonal_projection_operator_in_terms_of_reduced_incidence_matrices_and_sparse_R_factors} versus the left is that it requires only the computation of the R-factor $R$ of the matrix $\redIncMat(\directed{G})\transpose$, followed by a pair of triangular linear solves with $R$ and $R\transpose$ as the coefficient matrices;  each of these operations can be done efficiently since $\redIncMat(\directed{G})$ is generally quite sparse in practice.  We summarize this approach to computing $\OrthoProjMatrix$ as Algorithm \ref{algorithm_computing_the_matrix_of_the_orthogonal_projection_operator}.

% 
% 
% \begin{algorithm}[t]
% \caption{Computing the orthogonal projection matrix $\OrthoProjMatrix$}
% \label{algorithm_computing_the_matrix_of_the_orthogonal_projection_operator}
% \begin{algorithmic}[1]
% \Input The reduced incidence matrix $\redIncMat(\directed{G})$ of a weakly-connected directed graph $\directed{G}$.
% \Output The matrix $\OrthoProjMatrix$ of the orthogonal projection operator $\OrthoProj \colon \R^m \to \cycSpace(\directed{G})$ onto the directed cycle space of $\directed{G}$.
% \State  Compute the R-factor $R$ of a QR decomposition of $\redIncMat(\directed{G})\transpose$.
% \State Compute matrix $M_1$ as the solution of the sparse lower-triangular system $R\transpose M_1 = \redIncMat(\directed{G})$.
% \State Compute matrix $M_2$ as the solution of the sparse upper-triangular system $R M_2 = M_1$.
% \State Compute the orthogonal projector $P = \redIncMat(\directed{G})\transpose M_2$ onto the directed cut space of $\directed{G}$.
% \State \Return $\OrthoProjMatrix = I_m - P$.
%  \end{algorithmic}
% \end{algorithm}
% 
% \subsection{The complete graph}
% In this subsection, we compute the matrix $\OrthoProjMatrix$ of the orthogonal projection $\OrthoProj \colon \R^{n \choose 2} \to \cycSpace(\directed{K}_n)$ onto the directed cycle space of an orientation of the complete graph $K_n$ on $n$ vertices.  The main technical result we will employ is the following:
% \begin{lem}
% \label{pseudoinverse_of_incidence_matrix_of_orientation_of_complete_graph_lemma}
% Let $\directed{K}_n = (\Nodes, \dEdges)$ be an orientation of the complete graph $K_n$ on $n$ vertices.  Then the pseudoinverse of its incidence matrix is given explicitly by:
% \begin{equation}
% \label{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix}
% \begin{split}
% A(\directed{K}_n)\pinv &\in \R^{{n \choose 2} \times n}, \\
% A(\directed{K}_n)\pinv_{ei} &=
% \begin{cases}
% \frac{1}{n}, & e \in \inEdges(i), \\
% - \frac{1}{n}, & e \in \outEdges(i), \\
% 0, & e \notin \incEdges(i).
% \end{cases}
% \end{split}
% \end{equation}
% \end{lem}
% 
% \begin{proof}
% We will simply verify that the matrix $X \in \R^{ {n \choose 2} \times n}$ whose elements are determined by the right-hand side of \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix} satisfies the four criteria defining the (unique) Moore-Penrose pseudoinverse of $A \triangleq \incMat(\directed{K}_n)$ \cite[pg.\ 257]{Golub1996Matrix}:
% \begin{enumerate}
%  \item [(i)]  $AXA = A$;
%  \item [(ii)]  $XAX = X$;
%  \item [(iii)]  $(A X)\transpose = AX$;
%  \item [(iv)]  $(X A)\transpose = XA$.
% \end{enumerate}
% To that end, define the product $P\triangleq XA \in \R^{ {n \choose 2} \times {n \choose 2}}$ (with rows and columns indexed by the edges $\dEdges$), and consider the $ef$-element:
% \begin{equation}
% \label{elements_of_P_for_pseudoinverse_proof}
%  P_{ef} = \sum_{v \in \Nodes} X_{ev} A_{ve}.
% \end{equation}
% It follows from \eqref{incidence_matrix_definition} and \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix} that $X_{ev} A_{ve} \ne 0$ only if $e,f \in \delta(v)$.  Now if $e = f = (i,j)$, then
% \begin{equation}
% P_{ee} = \sum_{v \in \Nodes} X_{ev} A_{ve} = X_{ei} A_{ie} + X_{ej} A_{je} = \left(-\frac{1}{n}\right)(-1) + \left(\frac{1}{n}\right)(1) = \frac{2}{n}.
% \end{equation}
% On the other hand, if $e \ne f$ then $e$ and $f$ are incident on at most one common vertex, say $w$, and therefore the only nonzero term in the sum \eqref{elements_of_P_for_pseudoinverse_proof} is $X_{ew}A_{we}$, whose value is determined  by the relative orientations of the edges $e$ and $f$ (i.e.\ whether or not they are both oriented into or out of vertex $w$, cf.\   \eqref{incidence_matrix_definition} and \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix}).  We therefore have:
% \begin{equation}
% \label{definition_of_P_for_pseudoinverse_proof}
% \begin{split}
%  P & = XA, \\
%  P_{ef} &= 
%  \begin{cases}
%  \frac{2}{n}, & e = f,\\
%  \frac{1}{n}, & t(e) = t(f) \textnormal{  or  } h(e) = h(f), \\
%  -\frac{1}{n}, & t(e) = h(f) \textnormal{  or  } h(e) = t(f), \\
%  0, &\textnormal{otherwise}.
%  \end{cases}
%  \end{split}
% \end{equation}
% It is immediate from \eqref{definition_of_P_for_pseudoinverse_proof} that $P$ is symmetric, and therefore condition (iv) is satisfied.  Similarly, define $Q = AX \in \R^{n \times n}$ (with rows and columns indexed by the vertices $\Nodes$), and consider:
% \begin{equation}
% \label{elements_of_Q_for_pseudoinverse_proof}
% Q_{ij} = \sum_{e \in \dEdges} A_{ie} X_{ej}.
% \end{equation}
% 
% We observe that $A_{ie} X_{ej} \ne 0$ only if $e$ is incident on both $i$ and $j$.  Now if $i = j$, then $A_{ie} X_{ei} = \frac{1}{n}$ by \eqref{incidence_matrix_definition} and \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix}, and there are precisely $\deg(i) = n-1$ such nonzero terms in the sum \eqref{elements_of_Q_for_pseudoinverse_proof} since $\directed{K}_n$ is an orientation of the complete graph; this shows that $Q_{ii} = \frac{n-1}{n}$ for all $i \in \Nodes$.  On the other hand, for $i \ne j$ then $e = (i,j)$ or $e = (j,i)$ and $A_{ie}X_{ej} = - \frac{1}{n}$ is the only nonzero term in the sum \eqref{elements_of_Q_for_pseudoinverse_proof}.  We therefore have:
% \begin{equation}
%  \begin{split}
%  Q &= AX, \\
%  Q_{ij} &= 
%  \begin{cases}
%  \frac{n-1}{n}, & i = j, \\
%  -\frac{1}{n}, & i \ne j.
%  \end{cases}
%  \end{split}
% \end{equation}
% Again we observe that $Q$ is symmetric, and therefore condition (iii) is satisfied.  
% 
% Now define the product $U \triangleq QA = AXA \in \R^{n \times {n \choose 2}}$ with rows indexed by the vertices $\Nodes$ and columns indexed by the edges $\dEdges$, and consider the $ie$-element:
% \begin{equation}
% \label{elements_of_U_for_pseudoinverse_proof}
%  U_{ie} = \sum_{j \in \Nodes} Q_{ij} A_{je}.
% \end{equation}
% We observe that $A_{je} \ne 0$ only for $e \in \incEdges(j)$, and therefore \eqref{elements_of_Q_for_pseudoinverse_proof} simplifies as:
% \begin{equation}
% \label{final_elements_of_U_for_pseudoinverse_proof}
%  U_{ie} = Q_{it(e)} A_{t(e)e} + Q_{ih(e)} A_{h(e)e} = 
%  \begin{cases}
% 1, & e \in \inEdges(i), \\
% -1, & e \in \outEdges(i),\\
% 0, & \textnormal{otherwise},
%  \end{cases}
% \end{equation}
% by virtue of \eqref{elements_of_Q_for_pseudoinverse_proof} and \eqref{incidence_matrix_definition}.  Comparing \eqref{final_elements_of_U_for_pseudoinverse_proof} with \eqref{incidence_matrix_definition} shows that $U = QA = AXA = A$, which is condition (i).
% 
% Finally, define the product $V \triangleq PX = XAX \in \R^{{n \choose 2} \times n}$ with rows indexed by the edges $\dEdges$ and columns indexed by the vertices $\Nodes$, and consider the $ei$-element:
% \begin{equation}
% \label{elements_of_V_for_pseudoinverse_proof}
%  V_{ei} = \sum_{f \in \dEdges} P_{ef} X_{fi} = P_{ee} X_{ei} + \sum_{f \ne e} P_{ef}X_{fi}.
% \end{equation}
% Now
% \begin{equation}
% \label{diagonal_term_in_V}
%  P_{ee} X_{ei} =
%  \begin{cases}
% \frac{2}{n^2}, & e \in \inEdges(i), \\
% -\frac{2}{n^2}, & e \in \outEdges(i),
%  \end{cases}
% \end{equation}
% by \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix} and \eqref{definition_of_P_for_pseudoinverse_proof}.  Similarly, $P_{ef} X_{fi} \ne 0$ only if $e,f \in \incEdges(i)$, in which case
% \begin{equation}
%  \label{off_diagonal_term_in_V}
%  P_{ef} X_{ei} = 
%  \begin{cases}
% \frac{1}{n^2}, & e \in \inEdges(i), \\
% -\frac{1}{n^2}, & e \in \outEdges(i).
%  \end{cases}
% \end{equation}
% Since there are exactly $\deg(i) - 1 = n - 2$ nonzero terms in the summation on the right-hand side of \eqref{elements_of_V_for_pseudoinverse_proof}, we can simplify this expression for $V_{ei}$ as:
% \begin{equation}
% \label{simplified_elements_of_V_for_pseudoinverse_proof}
%  V_{ei} = 
%  \begin{cases}
% \frac{1}{n}, & e \in \inEdges(i), \\
% -\frac{1}{n}, & e \in \outEdges(i), \\
% 0, & e \notin \incEdges(i).
%  \end{cases}
% \end{equation}
% Comparing \eqref{equation_for_elements_of_pseudoinverse_of_complete_graph_incidence_matrix} and \eqref{simplified_elements_of_V_for_pseudoinverse_proof} shows that $V = PX = XAX = X$, which is condition (ii).  We therefore conclude that $X = A\pinv$, as claimed.
% \end{proof}
% 
% 
% \begin{cor}[The matrix of the orthogonal projection operator onto $\cycSpace(\directed{K}_n)$]
%  Let $\directed{K}_n = (\Nodes, \dEdges)$ be an orientation of the complete graph $K_n$ on $n$ vertices.  Then the matrix $\OrthoProjMatrix \in \R^{{n \choose 2} \times {n \choose 2}}$ of the orthogonal projection operator $\OrthoProj \colon \R^{n \choose 2} \to \cycSpace(\directed{K}_n)$ onto the directed cycle space of $\directed{K}_n$ is given by:
%  \begin{equation}
%   \label{elements_of_orthogonal_projection_operator_onto_cycle_space_of_complete_graph}
%   \begin{split}
%   \OrthoProjMatrix &\in \R^{{n \choose 2} \times {n \choose 2}}, \\
%   \OrthoProjMatrix_{ef} &= 
%  \begin{cases}
%  \frac{n-2}{n}, & e = f,\\
%  -\frac{1}{n}, & t(e) = t(f) \textnormal{  or  } h(e) = h(f), \\
%  \frac{1}{n}, & t(e) = h(f) \textnormal{  or  } h(e) = t(f), \\
%  0, &\textnormal{otherwise}.
%  \end{cases}
%  \end{split}
%  \end{equation}
% \end{cor}
% \begin{proof}
% Equation \eqref{matrix_of_orthogonal_projection_operator_onto_cycle_space} shows that $\OrthoProjMatrix = I_{n \choose 2} - \incMat(\directed{K}_n)\pinv\incMat(\directed{K}_n)$, and we have already computed the elements of this latter product in equation \eqref{definition_of_P_for_pseudoinverse_proof} as part of the proof of Lemma \ref{pseudoinverse_of_incidence_matrix_of_orientation_of_complete_graph_lemma}.
% \end{proof}
% 


==> figures/table.tex <==
%==================================================================== 
\sphere & $1.2782\e{6}$  & $5.8019\e{2}$  & $5.7595\e{2}$  & $5.7594\e{2}$ &$3.00$ & $31$ & $6.95$ & $1.86$ \\ 
\hline 
%==================================================================== 
\sphereHard & $1.0824\e{8}$  & $3.0413\e{6}$  & $1.2486\e{6}$  & $1.2485\e{6}$ &$3.00$ & $16$ & $3.61$ & $1.42$ \\ 
\hline 
%==================================================================== 
\torus & $1.8861\e{6}$  & $2.7666\e{4}$  & $1.2114\e{4}$  & $1.2114\e{4}$ &$3.00$ & $46$ & $24.50$ & $5.21$ \\ 
\hline 
%==================================================================== 
\grid & $7.2175\e{7}$  & $2.7465\e{5}$  & $4.2161\e{4}$  & $4.216\e{4}$ &$3.00$ & $49$ & $132.44$ & $18.05$ \\ 
\hline 
%==================================================================== 
\garage & $8.3617\e{3}$  & $6.2997\e{-1}$  & $6.2995\e{-1}$  & $6.2994\e{-1}$ &$3.00$ & $86$ & $203.30$ & $11.79$ \\ 
\hline 
%==================================================================== 
\cubicle & $2.7564\e{6}$  & $6.2484\e{2}$  & $6.2481\e{2}$  & $6.2481\e{2}$ &$3.00$ & $23$ & $181.12$ & $28.85$ \\ 
\hline 
%==================================================================== 
\rim & $4.116\e{7}$  & $1.6985\e{4}$  & $1.235\e{4}$  & $4.2699\e{4}$ &$3.00$ & $36$ & $651.89$ & $91.64$ \\ 
\hline 
%==================================================================== 


==> figures/tableIter_line_ave.tex <==
$21.39$ & $20.51$ & $19.54$ & $18.00$ \\ 


==> figures/tableIter_line_max.tex <==
$49$ & $32$ & $31$ & $31$ \\ 


==> figures/tableIter_line_min.tex <==
$16$ & $16$ & $15$ & $10$ \\ 

